Single-RF Multi-User Communication Through Reconfigurable Intelligent Surfaces: An Information-Theoretic Analysis

Reconfigurable intelligent surfaces (RISs) are typically used in multi-user systems to mitigate interference among active transmitters. In contrast, this paper studies a setting with a conventional active encoder as well as a passive encoder that modulates the reflection pattern of the RIS. The RIS hence serves the dual purpose of improving the rate of the active encoder and of enabling communication from the second encoder. The capacity region is characterized, and information-theoretic insights regarding the trade-offs between the rates of the two encoders are derived by focusing on the high- and low-power regimes.

==> packages_commands_theorems.tex <==

\usepackage[utf8]{inputenc} 


\usepackage[T1]{fontenc}


\usepackage{cite}

\usepackage[colorlinks = true]{hyperref}


\ifCLASSINFOpdf
 \usepackage[pdftex]{graphicx}
 \graphicspath{{../pdf/}{../jpeg/}}
 \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
\else
 \usepackage[dvips]{graphicx}
 \graphicspath{{../eps/}}
 \DeclareGraphicsExtensions{.eps}
\fi



\usepackage[cmex10]{amsmath}  
\DeclareMathOperator*{\argmax}{arg\,max} 
\DeclareMathOperator*{\argmin}{arg\,min}  
\usepackage{amssymb}
\interdisplaylinepenalty=2500



\usepackage{algorithmic}


\usepackage{array}


\usepackage{stfloats}

\usepackage{flafter}


\usepackage{url}


\usepackage{cases}


\usepackage{tikz}
\usetikzlibrary{calc} 
\usepackage{pgfplots}
\usetikzlibrary{patterns}
\usetikzlibrary{positioning}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{shapes} 
\usetikzlibrary{shapes.geometric} 
\usetikzlibrary{fit} 

\RequirePackage{microtype}

\usepackage{xcolor}
\definecolor{TechnionBlue}{rgb}{0, 0.1765, 0.3843} 
\definecolor{OliveGreen}{rgb}{0.4, 0.62, 0.25} 


\usepackage{ifthen}



\usepackage[normalem]{ulem}


\usepackage{fontawesome}



\newcommand{\rb}[1] {\left(#1\right)}
\newcommand{\cb}[1] {\left\lbrace #1 \right\rbrace}
\newcommand{\sqb}[1] {\left[#1\right]}
\newcommand{\given}[1]{\left\lvert#1\right.}
\newcommand{\AgivenB}[2]{\left(#1\middle\vert#2\right)}
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand*{\QEDA}{\hfill\ensuremath{\blacksquare}}
\newcommand*{\nspace}[1] {
	\ifthenelse{\equal{#1}{!}}{\!}{}
	\ifthenelse{\equal{#1}{tq}}{\kern-1em}{} 
	\ifthenelse{\equal{#1}{mq}}{\mkern-18mu}{} 
}



\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}



\DeclareMathOperator{\tr}{tr}
